Genetic Classification of Populations using Supervised Learning

There are many instances in genetics in which we wish to determine whether two candidate populations are distinguishable on the basis of their genetic structure. Examples include populations which are geographically separated, case--control studies and quality control (when participants in a study have been genotyped at different laboratories). This latter application is of particular importance in the era of large scale genome wide association studies, when collections of individuals genotyped at different locations are being merged to provide increased power. The traditional method for detecting structure within a population is some form of exploratory technique such as principal components analysis. Such methods, which do not utilise our prior knowledge of the membership of the candidate populations. are termed \emph{unsupervised}. Supervised methods, on the other hand are able to utilise this prior knowledge when it is available. In this paper we demonstrate that in such cases modern supervised approaches are a more appropriate tool for detecting genetic differences between populations. We apply two such methods, (neural networks and support vector machines) to the classification of three populations (two from Scotland and one from Bulgaria). The sensitivity exhibited by both these methods is considerably higher than that attained by principal components analysis and in fact comfortably exceeds a recently conjectured theoretical limit on the sensitivity of unsupervised methods. In particular, our methods can distinguish between the two Scottish populations, where principal components analysis cannot. We suggest, on the basis of our results that a supervised learning approach should be the method of choice when classifying individuals into pre-defined populations, particularly in quality control for large scale genome wide association studies.

==> ISN_names <==
{\bf 3} {\bf Trinity College Dublin} Derek W. Morris, Colm
O'Dushlaine,Elaine Kenny, Emma M. Quinn, Michael Gill, Aiden
Corvin;{\bf Cardiff University} Michael C.O'Donovan, George K. Kirov,
Nick J. Craddock, Peter A. Holmans, Nigel M.Williams, Lucy Georgieva,
Ivan Nikolov, N. Norton, H. Williams, Draga Toncheva,Vihra Milanova,
Michael J. Owen; {\bf Karolinska Institutet/University of North
Carolina at Chapel Hill} Christina M. Hultman, Paul Lichtenstein, Emma
F.Thelander, Patrick Sullivan; {\bf University College London} Andrew
McQuillin, Khalid Choudhury, Susmita Datta, Jonathan Pimm, Srinivasa
Thirumalai, Vinay Puri, Robert Krasucki, Jacob Lawrence, Digby
Quested, Nicholas Bass, Hugh Gurling; {\bf University of Aberdeen}
Caroline Crombie, Gillian Fraser, Soh Leh Kuan, Nicholas Walker, David
St Clair; {\bf University of Edinburgh} Douglas H. R. Blackwood,
Walter J. Muir, Kevin A. McGhee, Ben Pickard, Pat Malloy, Alan
W. Maclean, Margaret Van Beck; {\bf Queensland Institute of Medical
Research} Naomi R. Wray, Peter M. Visscher, Stuart Macgregor;{\bf
University of Southern California} Michele T. Pato, Helena Medeiros,
Frank Middleton, Celia Carvalho, Christopher Morley, AymanFanous,
David Conti, James A. Knowles, Carlos Paz Ferreira, AntonioMacedo,
M. Helena Azevedo, Carlos N. Pato; {\bf Massachusetts General
Hospital} Jennifer L. Stone, Douglas M. Ruderfer, Manuel
A. R. Ferreira, {\bf Stanley Center for Psychiatric Research and Broad
Institute of MIT and Harvard} Shaun M. Purcell, Jennifer L. Stone,
Kimberly Chambert, Douglas M. Ruderfer, Finny Kuruvilla, Stacey
B. Gabriel, Kristin Ardlie, Mark J. Daly, Edward M. Scolnick, Pamela
Sklar.

==> PLOTS/graph_data/ploteig <==
#!/usr/bin/perl  -w 

### ploteig -i eigfile -p pops -c a:b [-t title] [-s stem] [-o outfile] [-x] [-k] [-g]  [-z sep]
use Getopt::Std ;
use File::Basename ;

## pops : separated  -x = make postscript and pdf  -z use another separator
##  -k keep intermediate files
## NEW if pops is a file names are read one per line

getopts('i:o:p:c:s:d:z:t:xkg',\%opts) ;
$postscmode = $opts{"x"} ;
$kflag = $opts{"k"} ;
$gflag = $opts{"g"} ;
$keepgreen = 1 if($gflag);
$keepflag = 1 if ($kflag) ;
$keepflag = 1 unless ($postscmode) ;

$zsep = ":" ;
if (defined $opts{"z"}) {
 $zsep = $opts{"z"} ;
 $zsep = "\+" if ($zsep eq "+") ;
}

$title = "" ;
if (defined $opts{"t"}) {
 $title = $opts{"t"} ;
}
if (defined $opts{"i"}) {
 $infile = $opts{"i"} ;
}
else {
 usage() ;
 exit 0 ;
}
open (FF, $infile) || die "can't open $infile\n" ;
@L = (<FF>) ;
chomp @L ;
$nf = 0 ;
foreach $line (@L) { 
 next if ($line =~ /\#/) ;
 @Z = split " ", $line ;
 $x = @Z ;
 $nf = $x if ($nf < $x) ;
}
# printf "## number of fields: %d\n", $nf ;
$popcol = $nf-1 ;


if (defined $opts{"p"}) {
 $pops = $opts{"p"} ;
}
else {
 die "p parameter compulsory\n" ;
}

$popsname = setpops ($pops) ;
# print "$popsname\n" ;

$c1 = 1; $c2 =2 ;
if (defined $opts{"c"}) {
 $cols = $opts{"c"} ;
 ($c1, $c2) = split ":", $cols ;
 die "bad c param: $cols\n" unless (defined $cols) ;
}

$stem = "$infile.$c1:$c2" ;
if (defined $opts{"s"}) {
 $stem = $opts{"s"} ;
}
$gnfile = "$stem.$popsname.xtxt" ;
 
if (defined $opts{"o"}) {
 $gnfile = $opts{"o"} ;
}


@T = () ; ## trash 
open (GG, ">$gnfile") || die "can't open $gnfile\n" ;
print GG "## " unless ($postscmode) ;
print GG "set terminal postscript color\n" ;
print GG "set title  \"$title\" \n" ; 
print GG "set xlabel  \"eigenvector $c1\" \n" ; 
print GG "set ylabel  \"eigenvector $c2\" \n" ; 
print GG "plot " ;
$np = @P ;
$lastpop = $P[$np-1] ;
$d1 = $c1+1 ;
$d2 = $c2+1 ;
foreach $pop (@P)  { 
 $dfile = "$stem:$pop" ;
 push @T, $dfile ;
 print GG " \"$dfile\" using $d1:$d2 title \"$pop\" " ;
 print GG ", \\\n" unless ($pop eq $lastpop) ;
 open (YY, ">$dfile") || die "can't open $dfile\n" ;
 foreach $line (@L) {
  next if ($line =~ /\#/) ;
  @Z = split " ", $line ;
  next unless (defined $Z[$popcol]) ;
  next unless ($Z[$popcol] eq $pop) ;
  print YY "$line\n" ;
 }
 close YY ;
}
print GG "\n" ;
print GG "## "  if ($postscmode) ;
print GG "pause 9999\n"  ;
close GG ;

if ($postscmode) { 
$psfile = "$stem.ps" ;

 if ($gnfile =~ /xtxt/) { 
  $psfile = $gnfile ;
  $psfile  =~ s/xtxt/ps/ ;
 }
system "gnuplot < $gnfile > $psfile" ;
unless($keepgreen) { &fixgreen($psfile); } # to fix the color green 
system "ps2pdf  $psfile " ;
}
unlink (@T) unless $keepflag ;

sub usage { 
 
print "ploteig -i eigfile -p pops -c a:b [-t title] [-s stem] [-o outfile] [-x] [-k]\n" ;  
print "-i eigfile     input file first col indiv-id last col population\n" ;
print "## as output by smartpca in outputvecs \n" ;
print "-c a:b         a, b columns to plot.  1:2 would be common and leading 2 eigenvectors\n" ;
print "-p pops        Populations to plot.  : delimited.   eg  -p Bantu:San:French\n" ;
print "## pops can also be a filename.  List populations 1 per line\n" ;
print "[-s stem]      stem will start various output files\n"  ;
print "[-o ofile]     ofile will be gnuplot control file.  Should have xtxt suffix\n"; 
print "[-x]           make ps and pdf files\n" ; 
print "[-k]           keep various intermediate files although  -x set\n" ;
print "[-g]           keep default green color scheme\n" ;
print "## nexessary if .xtxt file is to be hand edited\n" ;
print "[-t]           title (legend)\n" ;

print "The xtxt file is a gnuplot file and can be easily hand edited.  Intermediate files
needed if you want to make your own plot\n" ;

}

sub setpops {      
 my ($pops) = @_  ; 
 local (@a, $d, $b, $e) ; 

 if (-e $pops) {  
  open (FF1, $pops) || die "can't open $pops\n" ;
  @P = () ;
  foreach $line (<FF1>) { 
  ($a) = split " ", $line ;
  next unless (defined $a) ;
  next if ($a =~ /\#/) ;
  push  @P, $a ;
  }
  $out = join ":", @P ; 
  print "## pops: $out\n" ;
  ($b, $d , $e) = fileparse($pops) ;
  return $b ;
 }
 @P = split $zsep, $pops ;
 return $pops ;

}

sub fixgreen {
  ## a better green color for gnuplot (dark green)
  ## and yellow

  local(@a);

  my ($IN) = @_ ;
  my $T1 = "$IN.$$" ;
  # system "cp $IN $IN.bak" ;
  open (FF, $IN) || die "can't open $IN\n" ;
  open (YY, ">$T1") || die "can't open $T1\n" ;
  foreach $line (<FF>) {
    chomp $line ;
    ($a) = split " ", $line ;
    if ($a eq "/LT1")  {
      $line = "/LT1 { PL [4 dl 2 dl] .2 .4 0 DL } def" ;
    }
    if ($a eq "/LT5")  {
      $line = "/LT5 { PL [4 dl 2 dl]  1 .8 0 DL } def" ;
    }
    print YY "$line\n" ;
  }
  close FF ;
  close YY ;
  system "mv $T1 $IN" ;
  unlink $T1 ;
}


==> PLOTS/graph_ps/ploteig <==
#!/usr/bin/perl  -w 

### ploteig -i eigfile -p pops -c a:b [-t title] [-s stem] [-o outfile] [-x] [-k] [-g]  [-z sep]
use Getopt::Std ;
use File::Basename ;

## pops : separated  -x = make postscript and pdf  -z use another separator
##  -k keep intermediate files
## NEW if pops is a file names are read one per line

getopts('i:o:p:c:s:d:z:t:xkg',\%opts) ;
$postscmode = $opts{"x"} ;
$kflag = $opts{"k"} ;
$gflag = $opts{"g"} ;
$keepgreen = 1 if($gflag);
$keepflag = 1 if ($kflag) ;
$keepflag = 1 unless ($postscmode) ;

$zsep = ":" ;
if (defined $opts{"z"}) {
 $zsep = $opts{"z"} ;
 $zsep = "\+" if ($zsep eq "+") ;
}

$title = "" ;
if (defined $opts{"t"}) {
 $title = $opts{"t"} ;
}
if (defined $opts{"i"}) {
 $infile = $opts{"i"} ;
}
else {
 usage() ;
 exit 0 ;
}
open (FF, $infile) || die "can't open $infile\n" ;
@L = (<FF>) ;
chomp @L ;
$nf = 0 ;
foreach $line (@L) { 
 next if ($line =~ /\#/) ;
 @Z = split " ", $line ;
 $x = @Z ;
 $nf = $x if ($nf < $x) ;
}
# printf "## number of fields: %d\n", $nf ;
$popcol = $nf-1 ;


if (defined $opts{"p"}) {
 $pops = $opts{"p"} ;
}
else {
 die "p parameter compulsory\n" ;
}

$popsname = setpops ($pops) ;
# print "$popsname\n" ;

$c1 = 1; $c2 =2 ;
if (defined $opts{"c"}) {
 $cols = $opts{"c"} ;
 ($c1, $c2) = split ":", $cols ;
 die "bad c param: $cols\n" unless (defined $cols) ;
}

$stem = "$infile.$c1:$c2" ;
if (defined $opts{"s"}) {
 $stem = $opts{"s"} ;
}
$gnfile = "$stem.$popsname.xtxt" ;
 
if (defined $opts{"o"}) {
 $gnfile = $opts{"o"} ;
}


@T = () ; ## trash 
open (GG, ">$gnfile") || die "can't open $gnfile\n" ;
print GG "## " unless ($postscmode) ;
print GG "set terminal postscript color\n" ;
print GG "set title  \"$title\" \n" ; 
print GG "set xlabel  \"eigenvector $c1\" \n" ; 
print GG "set ylabel  \"eigenvector $c2\" \n" ; 
print GG "plot " ;
$np = @P ;
$lastpop = $P[$np-1] ;
$d1 = $c1+1 ;
$d2 = $c2+1 ;
foreach $pop (@P)  { 
 $dfile = "$stem:$pop" ;
 push @T, $dfile ;
 print GG " \"$dfile\" using $d1:$d2 title \"$pop\" " ;
 print GG ", \\\n" unless ($pop eq $lastpop) ;
 open (YY, ">$dfile") || die "can't open $dfile\n" ;
 foreach $line (@L) {
  next if ($line =~ /\#/) ;
  @Z = split " ", $line ;
  next unless (defined $Z[$popcol]) ;
  next unless ($Z[$popcol] eq $pop) ;
  print YY "$line\n" ;
 }
 close YY ;
}
print GG "\n" ;
print GG "## "  if ($postscmode) ;
print GG "pause 9999\n"  ;
close GG ;

if ($postscmode) { 
$psfile = "$stem.ps" ;

 if ($gnfile =~ /xtxt/) { 
  $psfile = $gnfile ;
  $psfile  =~ s/xtxt/ps/ ;
 }
system "gnuplot < $gnfile > $psfile" ;
unless($keepgreen) { &fixgreen($psfile); } # to fix the color green 
system "ps2pdf  $psfile " ;
}
unlink (@T) unless $keepflag ;

sub usage { 
 
print "ploteig -i eigfile -p pops -c a:b [-t title] [-s stem] [-o outfile] [-x] [-k]\n" ;  
print "-i eigfile     input file first col indiv-id last col population\n" ;
print "## as output by smartpca in outputvecs \n" ;
print "-c a:b         a, b columns to plot.  1:2 would be common and leading 2 eigenvectors\n" ;
print "-p pops        Populations to plot.  : delimited.   eg  -p Bantu:San:French\n" ;
print "## pops can also be a filename.  List populations 1 per line\n" ;
print "[-s stem]      stem will start various output files\n"  ;
print "[-o ofile]     ofile will be gnuplot control file.  Should have xtxt suffix\n"; 
print "[-x]           make ps and pdf files\n" ; 
print "[-k]           keep various intermediate files although  -x set\n" ;
print "[-g]           keep default green color scheme\n" ;
print "## nexessary if .xtxt file is to be hand edited\n" ;
print "[-t]           title (legend)\n" ;

print "The xtxt file is a gnuplot file and can be easily hand edited.  Intermediate files
needed if you want to make your own plot\n" ;

}

sub setpops {      
 my ($pops) = @_  ; 
 local (@a, $d, $b, $e) ; 

 if (-e $pops) {  
  open (FF1, $pops) || die "can't open $pops\n" ;
  @P = () ;
  foreach $line (<FF1>) { 
  ($a) = split " ", $line ;
  next unless (defined $a) ;
  next if ($a =~ /\#/) ;
  push  @P, $a ;
  }
  $out = join ":", @P ; 
  print "## pops: $out\n" ;
  ($b, $d , $e) = fileparse($pops) ;
  return $b ;
 }
 @P = split $zsep, $pops ;
 return $pops ;

}

sub fixgreen {
  ## a better green color for gnuplot (dark green)
  ## and yellow

  local(@a);

  my ($IN) = @_ ;
  my $T1 = "$IN.$$" ;
  # system "cp $IN $IN.bak" ;
  open (FF, $IN) || die "can't open $IN\n" ;
  open (YY, ">$T1") || die "can't open $T1\n" ;
  foreach $line (<FF>) {
    chomp $line ;
    ($a) = split " ", $line ;
    if ($a eq "/LT1")  {
      $line = "/LT1 { PL [4 dl 2 dl] .2 .4 0 DL } def" ;
    }
    if ($a eq "/LT5")  {
      $line = "/LT5 { PL [4 dl 2 dl]  1 .8 0 DL } def" ;
    }
    print YY "$line\n" ;
  }
  close FF ;
  close YY ;
  system "mv $T1 $IN" ;
  unlink $T1 ;
}


==> abstract.tex <==

There are many instances in genetics in which we wish to determine
whether two candidate populations are distinguishable on the basis of
their genetic structure. Examples include populations which are
geographically separated, case--control studies and quality control
(when participants in a study have been genotyped at different
laboratories). This latter application is of particular importance in
the era of large scale genome wide association studies, when
collections of individuals genotyped at different locations are being
merged to provide increased power. The traditional method for
detecting structure within a population is some form of exploratory
technique such as principal components analysis.  Such methods, which
do not utilise our prior knowledge of the membership of the candidate
populations. are termed \emph{unsupervised}. Supervised methods, on
the other hand are able to utilise this prior knowledge when it is
available.

In this paper we demonstrate that in such cases modern supervised
approaches are a more appropriate tool for detecting genetic
differences between populations. We apply two such methods, (neural
networks and support vector machines) to the classification of three
populations (two from Scotland and one from Bulgaria). The sensitivity
exhibited by both these methods is considerably higher than that
attained by principal components analysis and in fact comfortably
exceeds a recently conjectured theoretical limit on the sensitivity of
unsupervised methods. In particular, our methods can distinguish
between the two Scottish populations, where principal components
analysis cannot. We suggest, on the basis of our results that a
supervised learning approach should be the method of choice when
classifying individuals into pre-defined populations, particularly in
quality control for large scale genome wide association studies.

